Efficient Dataset Selection for Continual Adaptation of Generative Recommenders

Recommendation systems must continuously adapt to evolving user behavior, yet the volume of data generated in large-scale streaming environments makes frequent full retraining impractical. This work investigates how targeted data selection can mitigate performance degradation caused by temporal distributional drift while maintaining scalability. We evaluate a range of representation choices and sampling strategies for curating small but informative subsets of user interaction data. Our results demonstrate that gradient-based representations, coupled with distribution-matching, improve downstream model performance, achieving training efficiency gains while preserving robustness to drift. These findings highlight data curation as a practical mechanism for scalable monitoring and adaptive model updates in production-scale recommendation systems.

==> sections/monthly_experiments.tex <==
\newpage
%\section{Monthly Experiments}\label{apdx:monthly_results}

%In this section, we list experiment results for continual learning using monthly intervals instead of 6-month intervals

%\input{figures/results_ref_size_monthly}
%\input{tables/monthly_results}

==> tables/monthly_results.tex <==
\begin{table}[h]
\caption{Performance in monthly continuous learning setting (no training)}
\label{tab:monthy_no_train}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2405 & 0.2516 & 0.3643 & 0.4089 & 0.2048 \\
    03/2022: & 0.2338 & 0.2452 & 0.3547 & 0.4013 & 0.1989 \\
    04/2022: & 0.235 & 0.246 & 0.356 & 0.4005 & 0.2 \\
    05/2022: & 0.2321 & 0.2428 & 0.3514 & 0.3943 & 0.1976 \\
    06/2022: & 0.2298 & 0.2402 & 0.3477 & 0.3889 & 0.1954 \\
    07/2022: & 0.2236 & 0.2338 & 0.34 & 0.3812 & 0.1896 \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\caption{Performance in monthly continuous learning setting (full training)}
\label{tab:monthy_full_train}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2621 & 0.2726 & 0.3876 & 0.4301 & 0.2255 \\
    03/2022: & 0.2704 & 0.2796 & 0.3929 & 0.4306 & 0.2347 \\
    04/2022: & 0.2713 & 0.2838 & 0.3941 & 0.4454 & 0.236 \\
    05/2022: & 0.2672 & 0.2811 & 0.3877 & 0.4442 & 0.2332 \\
    06/2022: & 0.2821 & 0.294 & 0.4036 & 0.4534 & 0.2468 \\
    07/2022: & 0.2718 & 0.2861 & 0.3887 & 0.4471 & 0.239 \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\caption{Performance in monthly continuous learning setting (Random 0.5)}
\label{tab:monthy_random_0.5}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2523 & 0.2637 & 0.3724 & 0.4179 & 0.2176 \\
    03/2022: & 0.2496 & 0.2606 & 0.3685 & 0.413 & 0.2149 \\
    04/2022: & 0.2499 & 0.2629 & 0.3692 & 0.4219 & 0.2157 \\
    05/2022: & 0.2536 & 0.2686 & 0.3635 & 0.4232 & 0.2233 \\
    06/2022: & 0.2617 & 0.2763 & 0.3717 & 0.4304 & 0.2311 \\
    07/2022: & 0.254 & 0.2654 & 0.3778 & 0.4256 & 0.2179 \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\caption{Performance in monthly continuous learning setting (Random 0.2)}
\label{tab:monthy_random_0.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2419 & 0.2519 & 0.3683 & 0.4085 & 0.2052 \\
    03/2022: & 0.2398 & 0.2488 & 0.3606 & 0.3966 & 0.2045 \\
    04/2022: & 0.2403 & 0.2512 & 0.3606 & 0.4047 & 0.2054 \\
    05/2022: & 0.2407 & 0.2517 & 0.3603 & 0.4045 & 0.2060 \\
    06/2022: & 0.2429 & 0.2523 & 0.3665 & 0.4054 & 0.2068 \\
    07/2022: & 0.2368 & 0.2469 & 0.3562 & 0.3972 & 0.2023 \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\caption{Performance in monthly continuous learning setting (Random 0.1)}
\label{tab:monthy_random_0.1}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2358 & 0.2475 & 0.3579 & 0.4040 & 0.2007 \\
    03/2022: & 0.2356 & 0.2459 & 0.3498 & 0.3908 & 0.2025 \\
    04/2022: & 0.2351 & 0.2461 & 0.3544 & 0.3984 & 0.2006 \\
    05/2022: & 0.2365 & 0.2469 & 0.3554 & 0.3976 & 0.2019 \\
    06/2022: & 0.2416 & 0.2523 & 0.3542 & 0.3972 & 0.2096 \\
    07/2022: & 0.2196 & 0.2348 & 0.3309 & 0.3908 & 0.1887 \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\caption{Performance in monthly continuous learning setting (RepSim 0.5 with TopK sampling)}
\label{tab:monthy_repsim_0.5_topk}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2486 & 0.2592 & 0.3740 & 0.4166 & 0.2117 \\
    03/2022: & 0.2538 & 0.2633 & 0.3678 & 0.4061 & 0.2205 \\
    04/2022: & 0.2547 & 0.2662 & 0.3742 & 0.4216 & 0.2200 \\
    05/2022: & 0.2565 & 0.2694 & 0.3689 & 0.4214 & 0.2244 \\
    06/2022: & 0.2648 & 0.2752 & 0.3818 & 0.4250 & 0.2307 \\
    07/2022: & 0.2542 & 0.2673 & 0.3650 & 0.4182 & 0.2229 \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\caption{Performance in monthly continuous learning setting (RepSim 0.2 with TopK sampling)}
\label{tab:monthy_repsim_0.2_topk}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2426 & 0.2523 & 0.3678 & 0.4064 & 0.2059 \\
    03/2022: & 0.2390 & 0.2476 & 0.3572 & 0.3912 & 0.2040 \\
    04/2022: & 0.2385 & 0.2479 & 0.3596 & 0.3980 & 0.2028 \\
    05/2022: & 0.2422 & 0.2530 & 0.3539 & 0.3971 & 0.2099 \\
    06/2022: & 0.2420 & 0.2508 & 0.3576 & 0.3936 & 0.2077 \\
    07/2022: & 0.2353 & 0.2448 & 0.3493 & 0.3884 & 0.2015 \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\caption{Performance in monthly continuous learning setting (RepSim 0.2 with BotomK sampling)}
\label{tab:monthy_repsim_0.2_bottomk}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2388 & 0.2500 & 0.3609 & 0.4060 & 0.2037 \\
    03/2022: & 0.2352 & 0.2457 & 0.3574 & 0.3992 & 0.1998 \\
    04/2022: & 0.2352 & 0.2467 & 0.3543 & 0.4004 & 0.2006 \\
    05/2022: & 0.2380 & 0.2486 & 0.3578 & 0.4008 & 0.2032 \\
    06/2022: & 0.2486 & 0.2576 & 0.3619 & 0.3984 & 0.2157 \\
    07/2022: & 0.2386 & 0.2486 & 0.3560 & 0.3975 & 0.2041 \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\caption{Performance in monthly continuous learning setting (GradSim 0.2 with TopK sampling)}
\label{tab:monthy_gradsim_0.2_topk}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2476 & 0.2583 & 0.3690 & 0.4113 & 0.2128 \\  
    03/2022: & 0.2414 & 0.2515 & 0.3620 & 0.4019 & 0.2064 \\
    04/2022: & 0.2335 & 0.2468 & 0.3505 & 0.4032 & 0.2005 \\
    05/2022: & 0.2378 & 0.2507 & 0.3498 & 0.4009 & 0.2062 \\
    06/2022: & 0.2367 & 0.2489 & 0.3528 & 0.4032 & 0.2036 \\
    07/2022: & 0.2455 & 0.2551 & 0.3606 & 0.3997 & 0.2121 \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\caption{Performance in monthly continuous learning setting (GradSim 0.2 with BottomK sampling)}
\label{tab:monthy_gradsim_0.2_bottomk}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2421 & 0.2545 & 0.3545 & 0.4050 & 0.2101 \\
    03/2022: & 0.2283 & 0.2397 & 0.3545 & 0.4000 & 0.1918 \\
    04/2022: & 0.2387 & 0.2512 & 0.3536 & 0.4037 & 0.2061 \\
    05/2022: & 0.2408 & 0.2515 & 0.3584 & 0.4015 & 0.2066 \\
    06/2022: & 0.2499 & 0.2598 & 0.3641 & 0.4044 & 0.2167 \\
    07/2022: & 0.2413 & 0.2523 & 0.3579 & 0.4030 & 0.2075 \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\caption{Performance in monthly continuous learning setting (RepSim 0.5 with TopK sampling and reference set of size 1000)}
\label{tab:monthy_repsim_0.5_topk_ref_1000}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2431 & 0.2535 & 0.3654 & 0.4065 & 0.2075 \\
    03/2022: & 0.2402 & 0.2482 & 0.3589 & 0.3904 & 0.2052 \\
    04/2022: & 0.2416 & 0.2510 & 0.3602 & 0.3982 & 0.2070 \\
    05/2022: & 0.2373 & 0.2473 & 0.3565 & 0.3968 & 0.2026 \\
    06/2022: & 0.2326 & 0.2417 & 0.3578 & 0.3940 & 0.1956 \\
    07/2022: & 0.2313 & 0.2421 & 0.3453 & 0.3889 & 0.1983 \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\caption{Performance in monthly continuous learning setting (RepSim 0.5 with TopK sampling and reference set of size 1000)}
\label{tab:monthy_repsim_0.2_topk_ref_1000}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc}
    \toprule
    Date & NDCG@10 & NDCG@50 & HR@10 & HR@50 & MRR 0 \\
    \midrule
    02/2022: & 0.2311 & 0.2422 & 0.3499 & 0.3960 & 0.1966 \\
    03/2022: & 0.2319 & 0.2428 & 0.3477 & 0.3923 & 0.1983 \\
    04/2022: & 0.1027 & 0.1163 & 0.1815 & 0.2420 & 0.0817 \\
    05/2022: & 0.2271 & 0.2394 & 0.3376 & 0.3877 & 0.1955 \\
    06/2022: & 0.0022 & 0.0108 & 0.0045 & 0.0492 & 0.0045 \\
    07/2022: & 0.0044 & 0.0066 & 0.0092 & 0.0195 & 0.0040 \\
    \bottomrule
\end{tabular}
}
\end{table}
